From What to Which: Decoding Modifier Grounding in Frozen MLLMs

As Multimodal Large Language Models (MLLMs) can describe increasingly complex visual scenes, token-level grounding becomes crucial. Yet, when an MLLM generates "the yellow banana on the left", established grounding approaches focus on what is in the image ("banana"), overlooking tokens that help describe which instance is meant ("yellow", "left"). In this work, we ask whether frozen MLLM representations contain decodable grounding information about the referred instance across generated tokens, extending to modifiers such as attributes, spatial expressions, and relational/action terms. To address this question, we introduce OTTER, a lightweight supervised probe over frozen MLLM representations that uses Optimal Transport (OT) to align generated tokens with visual regions and produce compact grounding maps. Our results show that (i) instance-discriminative visual information can be decoded from modifier tokens, with the clearest evidence for spatial terms, but (ii) is not confined to them, as contextualized object nouns also carry referential information; (iii) the recovered grounding remains informative under context perturbations, while selected regions remain relevant to generation; and (iv) the learned OT-based grounding extends beyond the controlled setting to free generation and cross-dataset transfer.

==> images/protocol_figure.tex <==
\begin{figure*}[htbp]
\centering
\begin{tikzpicture}[scale=0.75,
    transform shape,
    font=\footnotesize,
    >=Latex,
    box/.style={
        rounded corners=2.5pt,
        draw=otterbrown!45,
        line width=0.55pt,
        fill=ottercream,
        inner sep=5pt,
        align=left
    },
    group/.style={
        box,
        text width=0.4\textwidth
    },
    arrow/.style={
        ->,
        line width=0.7pt,
        draw=otterbrown!70
    }
]

% ---------------------------------------------------------
% Central question
% ---------------------------------------------------------
\node[
    rounded corners=3pt,
    draw=otterbrown,
    line width=0.8pt,
    fill=ottersand!55,
    text width=\textwidth,
    align=center,
    inner sep=6pt,
    font=\small
] (central) at (0,0) {
    \textbf{\RQ}
};

% ---------------------------------------------------------
% Three boxes
% ---------------------------------------------------------

\node[group, anchor=north] (controlled) at (-6.2,-1.75) {
    {\bfseries\color{otterdark} Controlled grounding}\\[-1.5mm]
    {\color{otterbrown!45}\rule{\linewidth}{0.35pt}}\\[1mm]

    {\bfseries\color{otterblue} Q1}
    Does the full referring expression improve grounding over the object noun alone?\\[1mm]

    {\bfseries\color{otterblue} Q2}
    Which token types carry instance-discriminative grounding information?\\[1.5mm]

    % {\scriptsize\color{midgray}
    % RefCOCO / RefCOCO-MOD}
};

\node[group, anchor=north] (controls) at (0,-1.75) {
    {\bfseries\color{otterdark} Referential structure and validation}\\[-1.5mm]
    {\color{otterbrown!45}\rule{\linewidth}{0.35pt}}\\[1mm]

    {\bfseries\color{otterblue} Q3}
    Is referential information modifier-specific, or distributed across contextualized tokens?\\[1mm]

    {\bfseries\color{otterblue} Q4}
    Does grounding depend on the learned token--visual mapping?\\[1mm]

    {\bfseries\color{otterblue} Q5}
    Are the recovered regions relevant to generation?
};

\node[group, anchor=north] (generalization) at (6.2,-1.75) {
    {\bfseries\color{otterdark} Generalization}\\[-1.5mm]
    {\color{otterbrown!45}\rule{\linewidth}{0.35pt}}\\[1mm]

    {\bfseries\color{otterblue} Q6}
    Does grounding generalize to free generation?\\[1mm]

    {\bfseries\color{otterblue} Q7}
    Does the learned grounding geometry transfer across datasets?\\[1.5mm]

    % {\scriptsize\color{midgray}
    % COCO Caption / OpenPSG / RefCOCOg}
};

% ---------------------------------------------------------
% Arrows
% ---------------------------------------------------------

\coordinate (branch) at (0,-1.05);

\draw[
    line width=0.7pt,
    draw=otterbrown!70
] (central.south) -- (branch);

\draw[arrow]
    (branch) -| (controlled.north);

\draw[arrow]
    (branch) -- (controls.north);

\draw[arrow]
    (branch) -| (generalization.north);

\end{tikzpicture}
\caption{
{Overview of the evaluation protocol.}
% Controlled experiments first identify if full expressions improve grounding and which tokens encode instance-specific information (Q1--Q2). 
% Next, counterfactual and probing controls test the signal's distribution, the learned mapping's necessity, and its relevance to generation (Q3--Q5). 
% Finally, free-generation and cross-dataset settings evaluate generalization (Q6--Q7).
}
\label{fig:evaluation_protocol}
\end{figure*}

==> sections/results.tex <==
\section{Results}
\label{sec:results}

We organize the results following the evaluation protocol in Section~\ref{sec:protocols}.
We first establish controlled instance-level grounding and examine where the corresponding signal is represented (Q1--Q3). We then test the role of the learned token--visual mapping and the relevance of the recovered regions to generation (Q4--Q5). Finally, we evaluate generalization to unconstrained generation and cross-dataset transfer (Q6--Q7).

\subsection{Controlled Instance-Level Grounding (Q1--Q2)}
\label{sec:controlled_modifier_results}

\paragraph{Phrase versus noun-only generation.}
Table~\ref{tab:refcoco_controlled_generated_token_grounding} shows that grounding the full referring expression is more informative than grounding the object noun alone. 
This establishes that the linguistic context specifying an instance provides useful grounding information beyond the object category. 
Importantly, this phrase-level comparison does not establish that the additional information is localized specifically in modifier representations; we address that distinction at the token level in Q2--Q3.

\paragraph{Grounding across token categories.}
RefCOCO-MOD allows us to ask where instance-level visual information can be decoded within the generated expression. As shown in Table~\ref{tab:refcoco_controlled_generated_token_grounding_tam_comparison}, the learned probe recovers grounding information across several linguistic roles, with particularly strong results for object nouns and spatial modifiers, followed by attributes. Relational/action terms provide a weaker but consistent signal.
Function words also contain non-trivial target information under the supervised probe. We do not interpret this as independent lexical visual semantics; rather, it suggests that referential information may be distributed through contextualized token representations. This observation motivates Q3, where we test directly whether the referred instance is encoded specifically by modifiers or shared across tokens.

\begin{table}[htpb]
\centering

\begin{minipage}[t]{0.49\linewidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.95}

\caption{
Controlled RefCOCO grounding.
Full metrics are reported in Appendix~\ref{app:full_tables}.
}
\label{tab:refcoco_controlled_generated_token_grounding}

\resizebox{\linewidth}{!}{
\begin{tabular}{llcccc}
\toprule
Protocol & Method & Energy $\uparrow$ & Soft-IoU $\uparrow$
& IoU@0.4 $\uparrow$ & Ent. $\downarrow$ \\
\midrule
\multirow{3}{*}{Phrase}
& Semantic & 0.170 & 0.156 & 0.177 & 0.993 \\
& OTTER & \textbf{0.405} & \textbf{0.264} & 0.332 & \textbf{0.891} \\
& OTTER-R $\beta{=}0.3$ & 0.254 & 0.205 & \textbf{0.348} & 0.974 \\
\midrule
\multirow{3}{*}{Noun-only}
& Semantic & 0.162 & 0.147 & 0.168 & 0.993 \\
& OTTER & \textbf{0.310} & \textbf{0.189} & 0.229 & \textbf{0.907} \\
& OTTER-R $\beta{=}0.4$ & 0.205 & 0.166 & \textbf{0.264} & 0.983 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\linewidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.95}

\caption{
RefCOCO-MOD Soft-IoU comparison.
Differences report paired-bootstrap $95\%$ CIs.
}
\label{tab:refcoco_controlled_generated_token_grounding_tam_comparison}

\resizebox{\linewidth}{!}{
\begin{tabular}{lrrrl}
\toprule
Token group & $n$ & TAM & OTTER & $\Delta$ [95\% CI] \\
\midrule
Phrase
& 10834 & 0.118 & \textbf{0.342}
& $+0.224\ [0.221,\,0.228]$ \\
Nouns
& 15881 & 0.106 & \textbf{0.310}
& $+0.204\ [0.201,\,0.207]$ \\
Spatial
& 5021 & 0.061 & \textbf{0.304}
& $+0.243\ [0.238,\,0.248]$ \\
Attributes
& 2722 & 0.119 & \textbf{0.285}
& $+0.167\ [0.161,\,0.173]$ \\
Rel./action
& 516 & 0.077 & \textbf{0.172}
& $+0.095\ [0.082,\,0.110]$ \\
Function
& 5017 & 0.060 & 0.244
& $+0.184\ [0.179,\,0.189]$ \\
\bottomrule
\end{tabular}
}
\end{minipage}

\end{table}

\subsection{Distributed Referential Grounding and Context Dependence (Q3)}
\label{sec:distributed_grounding}

Q1--Q2 show that modifier states contain instance-level visual information, but not whether this information is specific to modifiers. We therefore test how referential information is distributed across contextualized tokens.

\paragraph{Counterfactual referent switching.}
On natural same-image counterfactual pairs, modifier maps reliably follow the intended same-category referent, but contextualized noun maps do so just as reliably and can be even more selective (Table~\ref{tab:counterfactual}). The same pattern holds in the stricter left/right subset. Thus, the linguistic distinction between \emph{what} and \emph{which} does not correspond to a strict noun--modifier separation in the internal representations: instance identity is distributed across contextualized token states. This pattern is clearest for spatial expressions; attribute contrasts are broadly consistent, while relational/action pairs are too sparse for a reliable conclusion (Table~\ref{tab:counterfactual_types}).

\paragraph{Visual and contextual dependence.}
Replacing the correct image with a blank or unrelated one weakens referential selectivity for both nouns and modifiers, showing that the shared signal is not purely linguistic. Context perturbations further reveal that this distribution is not uniform: function-word grounding depends strongly on the surrounding expression, whereas spatial modifiers remain comparatively robust (Table~\ref{tab:context_control}). Referential information is therefore shared across tokens, but different token classes depend on context to different degrees.

\paragraph{Referential information before the modifier.}
In free generation we isolate expressions where the noun is produced before the disambiguating spatial modifier. Even in this causal setting, noun states already contain significant information about the intended instance, while the subsequently generated modifier is more discriminative. This suggests that the \emph{what-to-which} transition can begin before the explicit modifier is generated and become sharper as the referring expression unfolds.

\subsection{Matched Probe Controls (Q4)}
\label{sec:control_probes}

The matched controls in Table~\ref{tab:control_probes} produce a substantial performance collapse when the learned token--visual projection is replaced by either raw feature similarity or a shuffled mapping. Thus, the observed grounding cannot be attributed simply to RIS supervision, the OT operator, or an immediately accessible cosine geometry in the frozen features. Instead, the results support a more specific claim: frozen Qwen representations contain referential information that can be recovered by a lightweight learned projection. Since that projection is itself trained with RIS supervision, we do not interpret this as evidence for a fully pre-existing grounding geometry.


\begin{table}[t!]
\centering

%
% ================= COLONNA DI SINISTRA =================
\begin{minipage}[t]{0.49\textwidth}
\centering

\caption{Counterfactual referent grounding. 
Target preference measures whether a token map favours the intended same-category instance over the paired distractor. 
Gap is the mean target-minus-distractor score.}
\label{tab:counterfactual}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llcccc}
\toprule
Subset & Visual input &
\multicolumn{2}{c}{Target pref. $\uparrow$} &
\multicolumn{2}{c}{Gap $\uparrow$} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & Mod. & Noun & Mod. & Noun \\
\midrule
All natural & Correct & .776 & .779 & .203 & .242 \\
& Blank   & .703 & .705 & .112 & .137 \\
& Wrong   & .714 & .717 & .121 & .146 \\
\midrule
Clean L/R   & Correct & .772 & .795 & .220 & .293 \\
& Blank   & .677 & .744 & .115 & .193 \\
& Wrong   & .705 & .749 & .131 & .204 \\
\bottomrule
\end{tabular}%
}


\vspace{5mm} % Spazio verticale tra le tabelle di sinistra

\caption{Mean deletion AUC by token group on RefCOCO-val ($\uparrow$) over three $200$-unit repeats.}
\label{tab:faithfulness_stratified}
\scriptsize
\setlength{\tabcolsep}{2.3pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{lccccc}
\toprule
Method & Phrase & Noun & Modifier & Spatial & Attribute \\
\midrule
Random          & 0.310 & 0.305 & 0.182 & 0.151 & 0.226 \\
Attention       & 0.386 & 0.383 & 0.202 & 0.147 & 0.281 \\
Center          & 0.317 & 0.318 & 0.194 & 0.147 & 0.266 \\
Semantic branch & 0.541 & \textbf{0.536} & 0.320 & 0.227 & \textbf{0.450} \\
OTTER           & 0.543 & 0.535 & 0.322 & \textbf{0.234} & 0.445 \\
OTTER-R $\beta{=}0.5$ & \textbf{0.546} & 0.545 & \textbf{0.324} & 0.231 & 0.456 \\
\bottomrule
\end{tabular}

\end{minipage}\hfill
% ================= COLONNA DI DESTRA =================
\begin{minipage}[t]{0.49\textwidth}
\centering

\caption{Counterfactual grounding by modifier type (correct visual input).}
\label{tab:counterfactual_types}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Modifier type & Pairs &
\multicolumn{2}{c}{Target pref. $\uparrow$} &
\multicolumn{2}{c}{Gap $\uparrow$} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & Mod. & Noun & Mod. & Noun \\
\midrule
Spatial     & 2578 & .775 & .778 & .202 & .237 \\
Attribute   & 173  & .786 & .769 & .197 & .244 \\
Rel./action & 3    & .833 & .833 & .306 & .219 \\
\bottomrule
\end{tabular}%
}

\vspace{2.5mm} % Spazio verticale 

\caption{Matched control probes on RefCOCO-val under the same OT/RIS training.}
\label{tab:control_probes}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{lcc}
\toprule
Probe & Learned projection? & Calibrated mIoU $\uparrow$ \\
\midrule
OTTER               & yes & \textbf{0.458} \\
Raw cosine          & no  & 0.130 \\
Shuffled projection & no  & 0.135 \\
\bottomrule
\end{tabular}

\vspace{2.5mm} % Spazio verticale

\caption{Normalized Energy-in-GT retention under context perturbation. 
Values are normalized by global median noun retention. 
In brackets $95\%$ bootstrap CIs.}
\label{tab:context_control}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{lcc}
\toprule
Token group & Scrambled & Isolated \\
\midrule
Nouns     & $1.000\ [0.99,\,1.01]$ & $1.000\ [0.98,\,1.02]$ \\
Spatial   & $0.982\ [0.97,\,0.99]$ & $\mathbf{1.077\ [1.05,\,1.10]}$ \\
Attribute & $0.942\ [0.93,\,0.96]$ & $0.914\ [0.87,\,0.96]$ \\
Function  & $0.939\ [0.93,\,0.95]$ & $0.597\ [0.57,\,0.63]$ \\
\bottomrule
\end{tabular}

\end{minipage}
\end{table}



% \begin{table}[htpb]
% \centering

% % --- Prima Riga (Tabelle 1 e 2) ---
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \caption{Counterfactual referent grounding. Target preference measures whether a token map favors the intended same-category instance over the paired distractor. Gap is the mean target-minus-distractor score.}
% \label{tab:counterfactual}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{llcccc}
% \toprule
% Subset & Visual input &
% \multicolumn{2}{c}{Target pref. $\uparrow$} &
% \multicolumn{2}{c}{Gap $\uparrow$} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% & & Mod. & Noun & Mod. & Noun \\
% \midrule
% All natural & Correct & .776 & .779 & .203 & .242 \\
% & Blank   & .703 & .705 & .112 & .137 \\
% & Wrong   & .714 & .717 & .121 & .146 \\
% \midrule
% Clean L/R   & Correct & .772 & .795 & .220 & .293 \\
% & Blank   & .677 & .744 & .115 & .193 \\
% & Wrong   & .705 & .749 & .131 & .204 \\
% \bottomrule
% \end{tabular}%
% }
% \end{minipage}\hfill
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \caption{Counterfactual grounding by modifier type under the correct visual input.}
% \label{tab:counterfactual_types}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lrrrrr}
% \toprule
% Modifier type & Pairs &
% \multicolumn{2}{c}{Target pref. $\uparrow$} &
% \multicolumn{2}{c}{Gap $\uparrow$} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% & & Mod. & Noun & Mod. & Noun \\
% \midrule
% Spatial     & 2578 & .775 & .778 & .202 & .237 \\
% Attribute   & 173  & .786 & .769 & .197 & .244 \\
% Rel./action & 3    & .833 & .833 & .306 & .219 \\
% \bottomrule
% \end{tabular}%
% }
% \end{minipage}

% \vspace{6mm} % Spazio verticale tra le due righe di tabelle

% % --- Seconda Riga (Tabelle 3 e 4) ---
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \caption{Normalized Energy-in-GT retention under context perturbation. Values are normalized by global median noun retention; brackets show $95\%$ bootstrap CIs.}
% \label{tab:context_control}
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \begin{tabular}{lcc}
% \toprule
% Token group & Scrambled & Isolated \\
% \midrule
% Nouns     & $1.000\ [0.99,\,1.01]$ & $1.000\ [0.98,\,1.02]$ \\
% Spatial   & $0.982\ [0.97,\,0.99]$ & $\mathbf{1.077\ [1.05,\,1.10]}$ \\
% Attribute & $0.942\ [0.93,\,0.96]$ & $0.914\ [0.87,\,0.96]$ \\
% Function  & $0.939\ [0.93,\,0.95]$ & $0.597\ [0.57,\,0.63]$ \\
% \bottomrule
% \end{tabular}
% \end{minipage}\hfill
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \caption{Matched control probes on RefCOCO-val. All variants share the same OT/RIS training and calibration; only the semantic projection differs.}
% \label{tab:control_probes}
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \begin{tabular}{lcc}
% \toprule
% Probe & Learned projection? & Calibrated mIoU $\uparrow$ \\
% \midrule
% OTTER               & yes & \textbf{0.458} \\
% Raw cosine          & no  & 0.130 \\
% Shuffled projection & no  & 0.135 \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \end{table}

\subsection{Model Relevance under Perturbation (Q5)}
\label{sec:faithfulness_results}

Deletion experiments provide complementary evidence that the recovered regions are relevant to the model's own token generation. Across token groups, removing regions prioritized by OTTER has a stronger effect than removing random, center-selected, or attention-selected regions (Table~\ref{tab:faithfulness_stratified}). The learned semantic branch behaves similarly under this intervention, indicating that the main distinction introduced by OT lies in the spatial structure and concentration of the recovered maps rather than in their perturbation sensitivity. We therefore interpret deletion as evidence of model relevance, rather than as a complete causal account of token generation.

% \begin{table}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2.3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{
% Deletion AUC by token group on RefCOCO-val.
% Higher is better; values are means over three $200$-unit subsampling repeats.
% }
% \label{tab:faithfulness_stratified}
% \begin{tabular}{lccccc}
% \toprule
% Method & Phrase & Noun & Modifier & Spatial & Attribute \\
% \midrule
% Random
% & 0.310 & 0.305 & 0.182 & 0.151 & 0.226 \\
% Attention
% & 0.386 & 0.383 & 0.202 & 0.147 & 0.281 \\
% Center
% & 0.317 & 0.318 & 0.194 & 0.147 & 0.266 \\
% Semantic branch
% & 0.541 & \textbf{0.536} & 0.320 & 0.227 & \textbf{0.450} \\
% OTTER
% & 0.543 & 0.535 & 0.322 & \textbf{0.234} & 0.445 \\
% OTTER-Residual $\beta{=}0.5$
% & \textbf{0.546} & 0.545 & \textbf{0.324} & 0.231 & 0.456 \\
% \bottomrule
% \end{tabular}
% \end{table}

\subsection{Generalization beyond the Controlled Setting (Q6--Q7)}
\label{sec:generalization_results}

\paragraph{Free generation (Q6).}
Table~\ref{tab:refcoco_openpsg_free_generation_tam_protocol} evaluates OTTER on unconstrained generated text grounding on COCO Caption and OpenPSG. Because TAM is zero-shot whereas OTTER is RIS-supervised, we do not interpret the comparison as an intrinsic ranking of attribution methods. Rather, the results show that the grounding learned from RefCOCO-derived supervision remains useful when the model generates unconstrained captions outside the controlled referring-expression setup.

\paragraph{Cross-dataset transfer (Q7).}
Table~\ref{tab:transfer_refcocog} shows that the learned token--region mapping remains effective when transferred to RefCOCOg without retraining. The improvement extends beyond phrase-level grounding to nouns, attributes, spatial expressions, and relational/action terms. Together, Q6 and Q7 indicate that OTTER is not restricted to the specific RefCOCO expression distribution used for probe supervision: the learned grounding geometry transfers both to unconstrained generation and to a different referring-expression dataset.

\begin{table}[htpb]
\centering
\begin{minipage}[t]{0.65\textwidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\captionof{table}{Generalization performance on unconstrained free-generation.
\textbf{Best} in bold, \underline{second-best} underlined.}
\label{tab:refcoco_openpsg_free_generation_tam_protocol}
\vspace{1.5mm}
\begin{tabular}{@{}llcccccc@{}}
\toprule
Data & Method & Thr. & Obj.~$\uparrow$ & Func. & F1~$\uparrow$ & Prec.~$\uparrow$ & Rec.~$\uparrow$ \\
\midrule
\multirow{4}{*}{COCO}
& OTTER   & Otsu  & 0.193 & 0.929 & 0.320 & \textbf{0.471} & 0.290 \\
& OTTER-R ($\beta{=}0.5$) & $0.5$ & \underline{0.273} & 0.864 & \textbf{0.415} & 0.424 & 0.504 \\
& TAM     & Otsu  & \textbf{0.278} & 0.778 & \underline{0.409} & 0.404 & \textbf{0.668} \\
& TAM     & $0.5$ & 0.255 & 0.869 & 0.395 & \underline{0.450} & \underline{0.539} \\
\midrule
\multirow{4}{*}{OpenPSG}
& OTTER   & Otsu  & 0.210 & 0.934 & 0.343 & \textbf{0.479} & 0.300 \\
& OTTER-R ($\beta{=}0.5$) & $0.5$ & \textbf{0.284} & 0.863 & \textbf{0.427} & 0.425 & \underline{0.524} \\
& TAM     & Otsu  & \underline{0.258} & 0.784 & \underline{0.388} & 0.385 & \textbf{0.644} \\
& TAM     & $0.5$ & 0.235 & 0.873 & 0.370 & \underline{0.428} & 0.515 \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.34\textwidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{6pt}
\captionof{table}{
RefCOCOg transfer without retraining, reported as thresholded mIoU. \textbf{Best} in bold.
}
\label{tab:transfer_refcocog}
\vspace{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
Evaluation group & TAM & OTTER \\
\midrule
Phrase
& 0.171 & \textbf{0.372} \\
Nouns
& 0.134 & \textbf{0.332} \\
Attributes
& 0.152 & \textbf{0.328} \\
Spatial modifiers
& 0.053 & \textbf{0.328} \\
Rel./action
& 0.077 & \textbf{0.208} \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table}

\section{Discussion and Limitations}
\label{sec:discussion}
\include{images/qualitatives_collage_manuscript}
